A Methodology for Automating Assurance Case Generation

Safety Case has become an integral component for safety-certification in various Cyber Physical System domains including automotive, aviation, medical devices, and military. The certification processes for these systems are stringent and require robust safety assurance arguments and substantial evidence backing. Despite the strict requirements, current practices still rely on manual methods that are brittle, do not have a systematic approach or thorough consideration of sound arguments. In addition, stringent certification requirements and ever-increasing system complexity make ad-hoc, manual assurance case generation (ACG) inefficient, time consuming, and expensive. To improve the current state of practice, we introduce a structured ACG tool which uses system design artifacts, accumulated evidence, and developer expertise to construct a safety case and evaluate it in an automated manner. We also illustrate the applicability of the ACG tool on a remote-control car testbed case study.

==> Activity.tex <==
\begin{table}[h!]
    \centering
    \setlength{\belowcaptionskip}{-6pt}
    \renewcommand{\arraystretch}{1.2}
       \footnotesize
    \begin{tabular}{|c|p{1.5cm}|p{3cm}|}
    \hline
    Component& Type & Activity\\
    \hline
    Camera & Hardware & capture images\\
    \rowcolor{Gray} IR-OptoCoupler & Hardware & measure RPM\\
    LIDAR & Hardware & measure distance \\
    \rowcolor{Gray} Lane Detection & Software & detect lanes\\
    Object detection & Software & detect objects\\
    \rowcolor{Gray} Current speed & software & calculate speed\\
    Current position & software & calculate position\\
    \rowcolor{Gray} Obstacle distance & software & measure obstacle distance\\
    Slip status & software & identify wheel slip\\
    \rowcolor{Gray} Curated Images & software & process raw images\\
    LEC steer & software & compute steer\\
    \rowcolor{Gray} OpenCV steer & software & compute steer\\
    Braking Manager & software & calculate reverse RPM\\
    \rowcolor{Gray} Driving Manager & software & calculate speed \& \newline steer RPM\\
    PWM Applicator & Hardware & apply PWM to GPIO\\
    \hline
    \end{tabular}
    \caption{Activity Table: captures the activity associated with DeepNNCar's different components. It also shows the mapping of the components to their physical types.}
    \label{Table:Activity}
    \vspace{-0.4em}
\end{table}


==> Function-table.tex <==
\begin{table*}[t]
    \centering
    \setlength{\belowcaptionskip}{-6pt}
    \renewcommand{\arraystretch}{1.2}
      \footnotesize
    \begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|p{2.5cm}|p{5cm}|}
    \hline
    Subsystems & Functions & Components & Hardware & Software\\
    \hline
    \rowcolor{Gray} Sensing Subsystem (S1) & Sensing with multiple modalities (F1) & Camera Module \newline LIDAR Module \newline IR Opto-Coupler Module \newline Decawave Module & Camera Sensor \newline 2D LIDAR HW \newline IR Opto-Coupler HW \newline Decawave Sensor & OpenCV Camera capture \newline LIDAR Firmware \newline Opto-coupler Interrupt SW \newline Decawave Firmware\\
    Detection Subsystem (S2) & Surroundings detection (F2) & Lane Detection Module \newline Object Detection Module & Raspberry Pi3 & OpenCV Lane Detection Algorithm \newline Mobilenet V2 CNN Object Detection Model\\
    \rowcolor{Gray} State Estimation \newline Subsystem (S3) & Vehicle state Estimation (F3) & Current Speed Module \newline Current Position Module \newline Slip Status Module & Raspberry Pi3 & RPM-Speed Conversion SW \newline Decawave Position Estimator SW \newline Slip Evaluator SW\\
     Control Subsystem (S4) & 1) Steer computations (F4) \newline 2) Emergency Braking Logic (F5) \newline 3) Drive Signal generation (PWM) (F6) & LEC Module \newline OpenCV Steer Module \newline Braking Manager Module \newline Driving Manager Module \newline PWM Applicator Module & Raspberry Pi3 & NVIDIA DAVE-II CNN Model \newline Lane-Steer converter SW \newline Reverse Polarity Generation Module \newline Steer-Speed Evaluation Module\\
    \hline
    \end{tabular}
    \caption{Mapping between operational subsystems to different hardware and software components of DeepNNCar. For each subsystem, there are various functions (or component modules) that have to be checked during the safety case generation.}
    \label{Table:F2C}
    \vspace{-0.4em}
\end{table*}


==> table.tex <==

\begin{table*}[h!]
    \centering
    \setlength{\belowcaptionskip}{-6pt}
    \renewcommand{\arraystretch}{1.2}
       \footnotesize
    \begin{tabular}{|p{3cm}|p{4cm}|p{4cm}|p{4cm}|p{6cm}|}
    \hline
    Sub-Goals & Requirements & Evidence & Assumptions\\
    \hline
    \rowcolor{Gray} Camera module captures \newline image of Leader car. (G1) & 1) Camera can capture the image \newline of leader car. \newline 2) Light intensity above min value & Camera Module returns a cap object. & 1) Light intensity above min value \newline 2) Leader car is within capture range (min,max) \newline 3) Camera is powered.\\
    LIDAR module Provides reliable distance of leader car. (G2) & LIDAR can capture distances of car \newline in range (min,max) and angle (min,max). & LIDAR returns distance in range (0, 12m), angle (0\textdegree, 359\textdegree). & 1) Leader car is within scan range. \newline 2) LIDAR scanning frequency matches inference time. \newline 3) LIDAR is powered\\
    \rowcolor{Gray} IR Opto-coupler module provides reliable RPM information. (G3) & RPM measurement is within threshold limits & RPM measure is within (10, 50) & 1) It is mounted accurately. \newline 2)It can be occluded by plastic piece on wheel.\newline 3)It is powered.\\ 
    Lane Detection module reliably detects lanes in images. (G4) & Returns lane segment information in range [min,max] & Returns lane object = (-1,0,1,2) in range (0.1, 1)m. & 1) Received frame with lanes. \newline 2) LD parameters are correct. \newline 3) No light glare on track.\\
    \rowcolor{Gray} Object Detection module reliably detects car in images. (G5) & Returns object information in range (min,max) & Returns object = 0 or 1 in range (0.1,1)m if object identified. & 1) Received frame with front Car. \newline 2) LD parameters are correct. \newline 3) No light glare on track.\\
    Current Speed Module reliably provides speed information. (G6) & Speed measurement is within range (0,max) & Speed value returned is in range (0,1)m/s. & 1)Receives reliable RPM value from Opto-coupler module. \newline 2) RPM-Speed conversion is correct.\\
    \rowcolor{Gray}Current Position module reliably provides position information. (G7) & Position information tells if car is in track boundary & Position value returned is in range (-1,0,1).\newline -1 = out of track \newline 0 = center of track \newline 1 = not in center & 1) Received frame with lanes. \newline 2) LD algorithm accurately detects lanes.\\
    Slip Status module provides accurate wheel slip information. (G8) & Inform quickly if slipping found & Speed measurement values are consistently out of (0,1)m/s range. & 1)Track surface is known. \newline 2) Opto-coupler module is working correctly.\\
    \rowcolor{Gray} LEC module can provide reliable steering information. (G9) & Steer value is in range [min,max]&Steer value returned is always within (-30\textdegree, 30\textdegree) or PWM(10,20). & 1) Receives frames with lanes from camera module. \newline 2) Trained deep-learning model weights are correct. \newline 3)Trained model has seen the track before.\\
    OpenCV Steer module can provide reliable steering information. (G10) & Steer value is in range [min,max] & Steer value returned is always within (-30\textdegree, 30\textdegree) or PWM(10,20). & 1) Receives frames with lanes from camera module. \newline 2) LD Module returns accurate lane values. \newline 3) Lane-steer conversion is correct.\\
    \rowcolor{Gray} Braking Manager module provides reliable braking information. (G11) & Provides correct reverse PWM value based on distance calculation & Calculates Reverse PWM value $R_{PWM} \leq V_{PWM}$ to slow the car \newline 2)$R_{PWM}$=15.55 to emergency stop the car. & 1) Slip stats information is correct. \newline 2) OD module and LIDAR information is correct.\\ 
    Driving Manager module provides reliable steer, acceleration, and braking PWM values. (G12) & PWM values are in range (min,max) & Acceleration PWM is within (15.58, 15.62). \newline Braking PWM is within [15.55, 15.59]. \newline Steer PWM is within (10,20). & 1)LEC, OpenCV steer Module provide accurate steer values. \newline 2) Position module correctly updates position. \newline 3) LIDAR provides accurate distances. \newline 4) OD module correctly detects leader car. \newline 5)Braking Manager computes correct braking value.\\
    \rowcolor{Gray} PWM applicator module updates values to gpio reliably. (G13) & PWM values should comply with the frequency/ duty cycle. & Speed PWM is in range (15.55, 15.62). \newline Steer PWM is in range (10, 20). & 1) Wiring to motors and GPIO done correctly. \newline 2) Raspberry Pi3 is powered.\\
    \hline 
    \end{tabular}
    \caption{The sub-goals of the different functions is shown along with its requirement, evidences and the assumptions under which they hold.}
    \label{Table:SafetyTable}
    \vspace{-0.4em}
\end{table*}

